Unsupervised Spoken Term Discovery on Untranscribed Speech

(Part of the abstract) In this thesis, we investigate the use of unsupervised spoken term discovery in tackling this problem. Unsupervised spoken term discovery aims to discover topic-related terminologies in a speech without knowing the phonetic properties of the language and content. It can be further divided into two parts: Acoustic segment modelling (ASM) and unsupervised pattern discovery. ASM learns the phonetic structures of zero-resource language audio with no phonetic knowledge available, generating self-derived "phonemes". The audio are labelled with these "phonemes" to obtain "phoneme" sequences. Unsupervised pattern discovery searches for repetitive patterns in the "phoneme" sequences. The discovered patterns can be grouped to determine the keywords of the audio. Multilingual neural network with bottleneck layer is used for feature extraction. Experiments show that bottleneck features facilitate the training of ASM compared to conventional features such as MFCC. The unsupervised spoken term discovery system is experimented with online lectures covering different topics by different speakers. It is shown that the system learns the phonetic information of the language and can discover frequent spoken terms that align with text transcription. By using information retrieval technology such as word embedding and TFIDF, it is shown that the discovered keywords can be further used for topic comparison.

==> approvalPage.tex <==
%% Define your committee members. If you have less than 6, simple delete/comment the unused lines

\newcommand{\committeeMemberOne}{Dr. Burdell, Advisor}
\newcommand{\committeeMemberOneDepartment}{School of Myths}
\newcommand{\committeeMemberOneAffiliation}{Georgia Institute of Technology}

\newcommand{\committeeMemberTwo}{Dr. Two}
\newcommand{\committeeMemberTwoDepartment}{School of Mechanical Engineering}
\newcommand{\committeeMemberTwoAffiliation}{Georgia Institute of Technology}

\newcommand{\committeeMemberThree}{Dr. Three}
\newcommand{\committeeMemberThreeDepartment}{School of Electrical Engineering}
\newcommand{\committeeMemberThreeAffiliation}{Georgia Institute of Technology}

\newcommand{\committeeMemberFour}{Dr. Four}
\newcommand{\committeeMemberFourDepartment}{School of Computer Science}
\newcommand{\committeeMemberFourAffiliation}{Georgia Institute of Technology}

\newcommand{\committeeMemberFive}{Dr. Five}
\newcommand{\committeeMemberFiveDepartment}{School of Public Policy}
\newcommand{\committeeMemberFiveAffiliation}{Georgia Institute of Technology}

\newcommand{\committeeMemberSix}{Dr. Six}
\newcommand{\committeeMemberSixDepartment}{School of Nuclear Engineering}
\newcommand{\committeeMemberSixAffiliation}{Georgia Institute of Technology}

\newcommand{\approvalDay}{11}
\newcommand{\approvalMonth}{January}
\newcommand{\approvalYear}{2000}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not edit these lines unless you wish to customize
% the template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{titlepage}
\begin{singlespacing}
\begin{center}

\textbf{\MakeUppercase{\thesisTitle}}\\
\vspace{10\baselineskip}

\end{center}
\vfill

%Define minipages, depending on how many authors there are
\ifdefined\committeeMemberFour

Approved by:
\vspace{2\baselineskip}		%adjust the number in front of "\baselineskip" for alignment

\begin{minipage}[b]{0.4\textwidth}
	
	\committeeMemberOne\\
	\committeeMemberOneDepartment\\
	\textit{\committeeMemberOneAffiliation}\\
	
	\committeeMemberTwo\\
	\committeeMemberTwoDepartment\\
	\textit{\committeeMemberTwoAffiliation}\\
	
	\committeeMemberThree\\
	\committeeMemberThreeDepartment\\
	\textit{\committeeMemberThreeAffiliation}\\
	
	\vspace{2\baselineskip}		%adjust the number in front of "\baselineskip" for alignment
	
\end{minipage}
\hspace{0.1\textwidth}
\begin{minipage}[b]{0.4\textwidth}
	
	\committeeMemberFour\\
	\committeeMemberFourDepartment\\
	\textit{\committeeMemberFourAffiliation}\\
	
	\ifdefined\committeeMemberSix
	\committeeMemberFive\\
	\committeeMemberFiveDepartment\\
	\textit{\committeeMemberFiveAffiliation}\\
	
	\committeeMemberSix\\
	\committeeMemberSixDepartment\\
	\textit{\committeeMemberSixAffiliation}\\
	
	Date Approved: \approvalMonth{} \approvalDay, \approvalYear
	\vspace{1\baselineskip}		%adjust the number in front of "\baselineskip" for alignment
	
	\else
	
	\committeeMemberFive\\
	\committeeMemberFiveDepartment\\
	\textit{\committeeMemberFiveAffiliation}\\
		
	Date Approved: \approvalMonth{} \approvalDay, \approvalYear
	\vspace{5\baselineskip}		%adjust the number in front of "\baselineskip" for alignment
	
	\fi
	
\end{minipage}

\else

\hspace{0.6\textwidth}
\begin{minipage}[b]{0.4\textwidth}
	
	Approved by:
	\vspace{2\baselineskip}		%adjust the number in front of "\baselineskip" for alignment
	
	\committeeMemberOne\\
	\committeeMemberOneDepartment\\
	\textit{\committeeMemberOneAffiliation}\\
	
	\committeeMemberTwo\\
	\committeeMemberTwoDepartment\\
	\textit{\committeeMemberTwoAffiliation}\\
	
	\committeeMemberThree\\
	\committeeMemberThreeDepartment\\
	\textit{\committeeMemberThreeAffiliation}\\
	
	\vspace{2\baselineskip}		%adjust the number in front of "\baselineskip" for alignment
	
	Date Approved: \approvalMonth{} \approvalDay, \approvalYear
	\vspace{\baselineskip}		%adjust the number in front of "\baselineskip" for alignment
	
\end{minipage}

\fi





\end{singlespacing}
\end{titlepage}


==> dedication.tex <==
% Define your dedication statement here

\newcommand{\yourDedication}{A great dedication goes here.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not edit these lines unless you wish to customize
% the template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{titlepage}
\begin{center}

\vspace*{\fill}
\yourDedication\\
\vspace*{\fill}

\end{center}
\end{titlepage}


==> epigraph.tex <==
% Define your quote and author for the epigraph here

\newcommand{\yourQuote}{A great quote to start the thesis}
\newcommand{\yourAuthor}{George P. Burdell}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not edit these lines unless you wish to customize
% the template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{titlepage}
\begin{center}

\vspace*{\fill}
\yourQuote\\
\textit{\yourAuthor}
\vspace*{\fill}

\end{center}
\end{titlepage}



==> vita.tex <==
\chapter*{Vita}
\addcontentsline{toc}{chapter}{Vita}  %add Vita section to Table of Contents
Vita may be provided by doctoral students only. The length of the vita is preferably one page. It may include the place of birth and should be written in third person. This vita is similar to the author biography found on book jackets.
